On the Optimality of Batch Policy Optimization Algorithms

Batch policy optimization considers leveraging existing data for policy construction before interacting with an environment. Although interest in this problem has grown significantly in recent years, its theoretical foundations remain under-developed. To advance the understanding of this problem, we provide three results that characterize the limits and possibilities of batch policy optimization in the finite-armed stochastic bandit setting. First, we introduce a class of confidence-adjusted index algorithms that unifies optimistic and pessimistic principles in a common framework, which enables a general analysis. For this family, we show that any confidence-adjusted index algorithm is minimax optimal, whether it be optimistic, pessimistic or neutral. Our analysis reveals that instance-dependent optimality, commonly used to establish optimality of on-line stochastic bandit algorithms, cannot be achieved by any algorithm in the batch setting. In particular, for any algorithm that performs optimally in some environment, there exists another environment where the same algorithm suffers arbitrarily larger regret. Therefore, to establish a framework for distinguishing algorithms, we introduce a new weighted-minimax criterion that considers the inherent difficulty of optimal value prediction. We demonstrate how this criterion can be used to justify commonly used pessimistic principles for batch policy optimization.

==> defensive.tex <==
In addition to the confidence-biased index algorithm, we also consider a \emph{defensive}
algorithm:%
\todoch{better name?} 

\todot{The below definition looks odd to me. When $(n_i)$ are large, then $\hat \Delta_1$ will be negative if $1$ is optimal.
The natural definition would max over all $j$, but then this is equivalent to the LCB algorithm.}
\todoch{Actually the estimated reward gap should be $\max\{0, \hat{\Delta}\}$. But directly minimize over $\hat{\Delta}$ should also be fine as Csaba suggested below. } 

\begin{align*}
\MoveEqLeft \cA(X)=\argmin_{i\in[k]}\ \hat{\Delta}_i, \text{ where for }i\in [k],\\
\hat \Delta_i &= \max_{j\neq i} \hat{\mu}_j +  \frac{\beta_\delta}{\sqrt{n_j}} - ( \hat{\mu}_i -  \frac{\beta_\delta}{\sqrt{n_i}}) \, ,
\end{align*}
and 
where $\beta_\delta$ is the same parameter as in the index algorithm that defines the confidence interval. 
The next result shows that the user of the defensive algorithm can reliably predict the regret suffered.
Compare this to that the pessimistic algorithm can reliably predict how much reward it will collect.

\begin{lemma}
\label{lem:estimated-reward-gap}
On the event when the confidence intervals in \eqref{eq:confidence-interval} do not fail,
for any $i\in [k]$, $\Delta_i \le \max(0, \hat \Delta_i)$.
\end{lemma}
\begin{proof}
Assume that the confidence intervals do not fail and let $i\in [k]$.
If $i$ is the index of an optimal arm, $\Delta_i=0$ and there is nothing to be proven.
Otherwise, note that for any $j\in [k]$,
$ \hat{\mu}_j +  \frac{\beta_\delta}{\sqrt{n_j}} - (\hat{\mu}_i - \frac{\beta_\delta}{\sqrt{n_i}})
 \ge \mu_j - \mu_i$.
 Taking the maximum over $j\ne i$, the right-hand side is equal to $\Delta_i$ while the left-hand side is $\hat \Delta_i$.
\end{proof}
This shows that $\max(0,\hat{\Delta}_i)$  controls the random simple regret, which means one can also view the defensive algorithm as a ``pessimistic algorithm" as it minimizes an upper bound on the simple regret. \todoc{should the algorithm minimize $\max(0,\hat \Delta_i)$? I'd say it does not matter whether we do this. When the intervals do not fail, $\hat \Delta_i<0$ means that $i$ is optimal.}

We now provide the instance-dependent regret upper bound of the defensive algorithm. 

\todot{has $n_{\min}$ been defined?}

\todot{Is there a reason to introduce the constant $\delta = c/n$ below rather than just adding $\delta$. I would re-write
the condition as $n_{\min} \geq \frac{72}{\Delta_{\min}^2} \log(k/\delta)$. 
I'm also curious whether such a strong assumption is needed. What about
$n_i \geq \frac{const}{\Delta_i^2} \log(k/\delta)$ for all $i$?}

\todot{Bound below is somehow incomparable to the previous bounds -- how do we expect this algorithm behaves relative to the others?}

\todob{This defensive algorithm as well as its bound looks deviate from the confident-biased algorithm family. We need a better motivation for this part. How about move this to conclusion or discussion section in the end of this paper to position the paper as potential future work? }

\begin{theorem}
 Let $s=\argmax_{i\neq a^*} {\mu}_i + {2\beta_\delta}/{\sqrt{n_i}}$ and $h=\argmin\{n_s, n_{a^*}\}$.  
    Let $c$ be some constant such that $\delta = {c}/{n}$ and $\log \frac{K}{\delta}\leq \Delta_{\text{min}} \sqrt{\frac{n_{\text{min}}}{72}}$.  
    The regret of the defensive algorithm is upper bounded by,
    \begin{align}
    R(\cA) \leq \sum_{i\neq a^*}\Delta_i e^{- \frac{n_h \Delta_i^2}{288}}+ \frac{c}{n}\, .
    \end{align}
\end{theorem}

==> extra.tex <==
%\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\EEE}[2]{\mathbb{E}_{#1}\left[#2\right]}

\newcommand{\alg}{\cA}
\newcommand{\Amm}{\alg_{\mathrm{mm}}}
\newcommand{\Alcb}{\alg_{\mathrm{LCB}}}
\newcommand{\Rg}{R}
\newcommand{\Rmm}{\Rg_{\mathrm{mm}}}
\newcommand{\Rimm}{\Rg_{\mathrm{imm}}}
\newcommand{\Radv}{\Rg_{\mathrm{adv}}}
\newcommand{\Rper}{\Rg_{\mathrm{per}}}
\newcommand{\per}{\mathtt{per}}
\newcommand{\Aset}{\cG}
\newcommand{\abs}[1]{\left\lvert#1 \right\rvert}
\newcommand{\Thetat}{\tilde{\Theta}}


%\newpage
\section{A Deterministic Setting}

\todoy[inline]{This actually gives insights for many questions since it enables exact calculation of many quantities...?}

to understand what is going on, e.g. what are the possible arguments for which algorithm we should use.

\subsection*{Problem Setup: Observing the True Parameters}

$1 \le n < k$ observations (samples). Each observation reveals the true $\theta_i$ for arm $i$. Each arm $i \in \iset{k}$ is observed at most once. Without loss of generality, we assume that the observed arms are $1,...,n$ and $\theta \in \Theta = [0, 1]^k$. We consider deterministic algorithms that maps observed $X = \theta_{1:n} = \left[\theta_1, ..., \theta_n\right]$ to an arm $\alg(X)\in \iset{k}$. 
Given an instance $\theta$, the regret for an arm $i$ is defined as $\Rg(i, \theta) = \theta^* - \theta_i$ where $\theta^* = \max_{i\in \iset{k}} \theta_i$, and the regret for an algorithm $\alg$ is defined as $\Rg(\alg, \theta) = \Rg(\alg(\theta_{1:n}), \theta) = \theta^* - \theta_{\alg(\theta_{1:n})}$.

\todoy[inline]{Do we just assume $n\le k - 2$ for simplicity? $n=k-1$ needs to be discussed separately in many statements.}

\subsection*{Possible Algorithms}

Index algorithms $\alg_{\alpha}$ with $\alpha\in [0, 1]$: 
Define $\hat{\theta}_i = X_i$ for $i\in \iset{n}$ and $\theta_i = \alpha$ for $i > n$. Then $\alg_{\alpha}(X) = \argmax_{i\in \iset{k}} \hat{\theta}_i$. Note that $\alpha=0$ and $\alpha=1$ lead to LCB and UCB algorithms respectively. 

We define the algorithm that implements the minimax strategy as $\Amm(X) = \argmin_i \max_{\theta:\theta_{1:n}=X} \Rg(i, \theta)$. Note that the LCB algorithm $\alg_{0}(X) = \argmin_i \max_{\theta:\theta_{1:n}=X} -\theta_i$, which also implements the minimax strategy with respect to the reward but not the regret. 

We assume that the algorithms pick the arm with the smaller index for tie breakers in $\argmin$ or $\argmax$.

\begin{remark}
When $n \le k - 2$, $\alg_0$ and $\Amm$ are the same algorithm where $\alg_0(X) = \Amm(X) = \argmax_{1\le i \le n}X_i$. When $n = k - 1$, $\Amm = \alg_{1/2}$. 
That is, $\Amm(X) = \argmax_{1\le i \le n}X_i$ if $\max_{1\le i \le n} X_i \ge 1/2$ and $\Amm(X) = k$ otherwise.
\end{remark}

\begin{proof}
$\alg_0(X) = \argmax_{1\le i \le n}X_i$ by definition. Now we consider $\Amm$. For $i\le n$, 
$\max_{\theta:\theta_{1:n}=X} \Rg(i, \theta) = 1 - X_i$ because setting $\theta_{n+1}=1$ maximizes $\Rg(i, \theta)$. 
When $n\le k-2$, for $i>n$, $\max_{\theta:\theta_{1:n}=X} \Rg(i, \theta) = 1$ because we can always set $\theta_i=0$ and $\theta_j=1$ for some $j>n, j\ne i$.Therefore, for $n \le k - 2$, $\Amm(X) = \argmax_{i\iset{n}} X_i$.
When $n = k-1$, for $i>n$~($i=k$), $\max_{\theta:\theta_{1:n}=X} \Rg(i, \theta) = \max_{i\in \iset{n}} X_i$ by setting $\theta_k=0$. Therefore, for $n \le k - 2$, $\Amm(X)=\argmax_{i\iset{n}} X_i$ if $1 - \max_{i\in \iset{n}} X_i \le \max_{i\in \iset{n}} X_i$~(i.e., $\max_{i\in \iset{n}} X_i \ge 1/2$), and $\Amm(X) = k$ otherwise.
\end{proof}

%\todoy[inline]{maybe look at results from game theory for the deterministic setting?}

We now derive the regret for different algorithms. The exact regret for index algorithms is:
\begin{align*}
\Rg(\alg_{\alpha}, \theta) = 
\begin{cases}
\theta^* - \theta_{1:n}^* & \textrm{ if } \theta_{1:n}^* \ge \alpha, \\
\theta^* - \theta_{n+1} & \textrm{ otherwise}. 
\end{cases}
\end{align*}
Here we define $\theta_{1:n}^*=\max_{i\in \iset{n}} \theta_i$.
$\Rg(\Amm, \theta) = \Rg(\alg_{0}, \theta)$ for $n\le k - 2$, and $\Rg(\Amm, \theta) = \Rg(\alg_{1/2}, \theta)$ for $n=k-1$.

Similar conclusion holds as in the stochastic setting.

\subsection*{Minimax Optimality}

\begin{proposition}
Let $\Rmm = \min_{\alg} \max_{\theta} \Rg(\alg, \theta)$. Then $\Rmm = 1$ for $n \le k-2$ and $\Rmm = 1/2$ for $n=k-1$. 
\end{proposition}

\begin{proof}
For $n\le k-2$, consider $\theta_1=...=\theta_n=0$ and $\theta_{k-1}, \theta_k$ can be either $0, 1$ and $1, 0$. Then any algorithm must suffer regret $1$ in at least one of these two instance.
When $n=k-1$, consider $\theta_1=...\theta_{k-1}=1/2$ and $\theta_k\in \{0, 1\}$.
Then any algorithm must suffer regret at least $1/2$ in one of these two instances. On the other hand, the algorithm $\Amm$
has worst case regret guarantee of $1/2$. Hence $1/2$ is the minimax value when $n=k-1$.
\end{proof}

For any constant $c\ge 1$, define
\begin{align*}
\Aset_c = \left\{\alg: \max_{\theta} \Rg(\alg, \theta) \le c \Rmm \right\}
\end{align*}
to be the set of algorithms that are minimax optimal up to a multiplicative constant factor $c$.

Now we characterize the minimax optimality for different algorithms.
\begin{proposition}
(i) For any algorithm $\alg$, we have $\alg \in \Aset_2$.
(ii) When $n\le k-2$, for any algorithm $\alg$ we have $\alg \in \Aset_1$. (iii) For $n=k-1$, among all index algorithms only $\alg_{1/2}=\Amm \in \Aset_1$.    
\end{proposition}
\begin{proof}
The first two statements are trivial. For $n=k-1$, if $\alpha<1/2$, let $\theta=[\frac{2\alpha+1}{4},...,\frac{2\alpha+1}{4}, 1]$ then the algorithm selects $\alg_{\alpha}\in \iset{k-1}$ thus $\Rg(\alg_{\alpha}, \theta) = \frac{3 - 2\alpha}{4} > 1/2$.  If $\alpha > 1/2$ let $\theta=[\frac{2\alpha+1}{4},...,\frac{2\alpha+1}{4}, 0]$ then the algorithm selects $\alg_{\alpha}=k$ thus $\Rg(\alg_{\alpha}, \theta) = \frac{2\alpha + 1}{4} > 1/2$.
\end{proof}


\subsection*{Instance-wise Optimality under the Minimax Optimality Constraint}

Define
$\Rimm(\theta) = \min_{\alg \in \Aset_c} R(\alg, \theta)$ to be the instance dependent lower bound for any algorithm that is minimax optimal up to a constant $c$. Then we have
\begin{proposition}
When $n\le k-2$ or $c\ge 2$, $\Rimm(\theta)=0$ for all $\theta$. When $n=k-1$ and $1\le c < 2$, let $\theta_{1:n}^*=\max_{i\in \iset{n}} \theta_i$. Then
\begin{align*}
\Rimm(\theta) = 
\begin{cases}
0 & \textrm{ if } \theta_{1:n}^* \in \left[1-\frac{c}{2}, \frac{c}{2}\right]\,, \\
\theta^* - \theta_k &  \textrm{ if } \theta_{1:n}^* < 1-\frac{c}{2}\,, \\
\theta^* - \theta_{1:n}^* & \textrm{ if } \theta_{1:n}^* > \frac{c}{2}\,. \\
\end{cases}
\end{align*}
\end{proposition}

\begin{proof}
When $n\le k-2$ or $c\ge 2$, $\Aset_c$ contains all algorithms. So for each instance $\theta$ any algorithm that chooses the best arm when observing $\theta_{1:n}$ achieve regret $0$.

For $n = k-1$ and $c \in [1, 2)$. We have $\Rmm=1/2$ and $\Aset_c = \left\{\alg: \max_{\theta} \Rg(\alg, \theta) \le c/2 \right\}$. Notice that $\theta^* = \max\{\theta_k, \theta^*_{1:n}\}$, i.e., the best arm is either the best observed arm or arm $k$. 
(i) When $\theta_{1:n}^* \in \left[1-\frac{c}{2}, \frac{c}{2}\right]$, an algorithm $\alg$ that selects $\alg(\theta_{1:n})\in \{\argmax_{i\in \iset{n}}\theta_i, k\}$ must satisfy $\max_{\theta':\theta'_{1:n}}R(\alg, \theta') \le c/2$. So given $\theta$ that satisfies $\theta_{1:n}^* \in \left[1-\frac{c}{2}, \frac{c}{2}\right]$, the algorithm $\alg$ defined by $\alg(\theta_{1:n})=\argmax_i \theta_i$ and $\alg(X)=\alg_{1/2}(X)$ otherwise satisfies both $\alg \in \Aset_c$ and $\alg(\theta)=0$. So $\Rimm(\theta)=0$.
(ii) When $\theta_{1:n}^* < 1 - c/2$, any algorithm $\alg \in \Aset_c$ must select arm $k$, otherwise we can let $\theta_k=1$ then $R(\alg, \theta) > c/2$. There exists an algorithm $\alg_{1/2} \in \Aset_c$ so $\Rimm(\theta)=\theta^*-\theta_k$. (ii) When $\theta_{1:n}^* > c/2$, any algorithm $\alg \in \Aset_c$ must not select arm $k$, otherwise we can let $\theta_k=0$ then $R(\alg, \theta) > c/2$. So $\Rimm(\theta)\ge \theta^*-\theta_{1:n}^*$. There exists an algorithm $\alg_{1/2} \in \Aset_c$ which achieves $R(\alg_{1/2}, \theta)=\theta^*-\theta_{1:n}*$ so $\Rimm(\theta)=\theta^*-\theta_{1:n}^*$.
\end{proof}


No algorithm is instance-wise optimal:
\begin{proposition}
For any $n\in \iset{k-1}$, $c\ge 1$, and any algorithm $\alg$, we have $\sup_{\theta} \frac{\Rg(\alg, \theta)}{\Rimm(\theta)} = +\infty$.~(Here we define $0/0=1$.)
\end{proposition}

\begin{proof}
Consider $\theta=\left[1/2,...,1/2,0 \right]$ and $\theta'=\left[1/2,...,1/2,1 \right]$. Then $\Rimm(\theta)=\Rimm(\theta')=0$ for all cases, including $n=k-1$. Since $\theta_{1:n}=\theta'_{1:n}$ any algorithm must output the same action for $\theta$ and $\theta'$, suffering $1/2$ regret in one of the two instances.
\end{proof}

\begin{remark}
For $n=k-1$ and $c=1$, the algorithm $\Amm = \alg_{1/2}$ is instance-wise optimal except for the instances where $\theta_k > \theta_{1:n}^*=1/2$. 
\end{remark}

\subsection*{Local minimax optimality}

\todoy[inline]{
discuss why do we care about this? what are the possible definitions, what are the differences between them, etc
}


\subsection*{Local minimax optimality I, the adversarial instance}

Define\todoy{add citation}
\begin{align*}
\Radv(\theta) = \max_{\lambda\in \Theta} \min_{\alg} \max\left\{\Rg(\alg, \lambda), \Rg(\alg, \theta) \right\} \,.
\end{align*}

\begin{proposition}
Given $\theta$ define $\theta_{n+1:k}^-=\min_{n+1\le i\le k} \theta_i$. Then
\begin{align*}
\Radv(\theta) = \max\big\{ & \min\left\{\theta_{1:n}^*, \theta^*-\theta_{1:n}^*\right\}, \\ 
 & \min\left\{1 - \theta_{1:n}^*, \theta^* - \theta_{n+1:k}^- \right\} \big\}\,. \addeq\label{eq:radv}
\end{align*}
\end{proposition}

\begin{proof}
First observe that we only need to consider $\lambda$ where $\lambda_{1:n}=\theta_{1:n}$ because otherwise the algorithm can just select the best arm in $\lambda$ and $\theta$ respectively and achieves $0$ regret in both instances. When $\lambda_{1:n}=\theta_{1:n}$, any algorithm will select the same arm in both $\lambda$ and $\theta$. So we can write $\Radv$ as
\begin{align*}
\Radv(\theta) = \max_{\lambda\in \Theta} \min_{i\in \iset{k}} \max\left\{\lambda^* - \lambda_i, \theta^* - \theta_i \right\} \,. 
\end{align*}
We now discuss how to find the corresponding $\lambda$ for $\theta$. We divide all $\lambda \in \Theta$ into two categories: $\lambda^* = \lambda_{1:n}^*$ and $\lambda^* > \lambda_{1:n}^*$.

...

\end{proof}

\begin{proposition}
discuss optimality:
For $n\le k-2$, $\sup_\theta \frac{\Rg(\alg_{\alpha}, \theta)}{\Radv(\theta)} = \max\{\frac{1-\alpha}{\alpha}, \frac{1}{1 - \alpha}\}$. For $n=k-1$, $\sup_\theta \frac{\Rg(\alg_{\alpha}, \theta)}{\Radv(\theta)} = \max\{\frac{1-\alpha}{\alpha}, \frac{\alpha}{1 - \alpha}\}$.
\end{proposition}

\begin{proof}
...
\end{proof}

The local minimax optimality does not favor the LCB algorithm $\alg_0$.
\begin{remark}
$\alg_{1/2}$ is optimal with respect to $\Radv$ up to a constant factor $2$: For $n\le k-2$, $\sup_\theta \frac{\Rg(\alg_{1/2}, \theta)}{\Radv(\theta)} = 2$. For $n=k-1$, $\sup_\theta \frac{\Rg(\alg_{1/2}, \theta)}{\Radv(\theta)} = 1$. The LCB algorithm $\alg_{0}$ is not optimal with respect to $\Radv$ up to any constant factor:
$\sup_\theta \frac{\Rg(\alg_{1/2}, \theta)}{\Radv(\theta)} = +\infty$.
\end{remark}

If we only consider $\theta$ that is away from the boundary, then any index algorithm is optimal with respect to $\Radv$.
\begin{proposition}
Let $\theta_{\min} = \min_{i\in \iset{k}}\theta_i$.
Define $\Theta'=\left\{ \theta: \theta^* - \theta_{\min} \le \min\{\theta_{\min}, 1 - \theta^*\} \right\}$. 
Then $\Rg(\alg_{\alpha}, \theta) \le \Radv(\theta)$ for all $\theta\in \Theta'$.
\end{proposition}

\begin{proof}
For $\theta\in \Theta'$, $\Radv(\theta) = \max\{\theta^* - \theta_{1:n}^*, \theta^* - \theta_{n+1:k}^-\}$ thus the statement holds.
\end{proof}

A special category of instances is where all the unseen arms are better than the observed ones.\todoy{what can we say about this category} If we exclude this category of instances, the LCB algorithm $\alg_0$ is more favorable, but only up to a factor of $2$ compared to $\alg_{1/2}$:
\begin{proposition}
Define $\Thetat=\left\{ \theta: \theta_{1:n}^* > \theta_{n+1:k}^- \right\}$. 
Then For $n\le k-2$, $\sup_{\theta \in \Thetat} \frac{\Rg(\alg_{\alpha}, \theta)}{\Radv(\theta)} = \frac{1}{1 - \alpha}$. For $n=k-1$, $\sup_{\theta \in \Thetat} \frac{\Rg(\alg_{\alpha}, \theta)}{\Radv(\theta)} = \max\{ \frac{\alpha}{ 1 - \alpha}, 1\}$.
\end{proposition}

\begin{proof}
...
\end{proof}



\subsection*{Local minimax optimality II, the permutation model}
\todoy[inline]{The result is not really minimax, but instance-wise}

Define
\begin{align*}
\Rper(\theta) = \min_{\alg} \max_{\lambda\in \per(\theta)}\Rg(\alg, \lambda) \,.
\end{align*}
where $\per(\theta)$ is the set of instances that is a permutation~(of the arm indices) of $\theta$. 

\begin{proposition}
Let $\theta_{(1)}\le \theta_{(2)} \le ,..., \le \theta_{(k)}$ be the sorted permutation of $\theta$, then
$\Rper(\theta) = \theta^* - \theta_{(n+1)}$.
\end{proposition}

\begin{proof}
...
\end{proof}

Instance dependent lower bound within $\per(\theta)$. Let $\Aset_{\per(\theta)} = \{\alg: \max_{\lambda\in \per(\theta)} \Rg(\alg, \lambda) \le \Rper(\theta)\}$ be the set of all minimax optimal algorithms with respect to $\per(\theta)$ and $\tilde{\Rg}_{\per}(\theta) = \min_{\alg \in \Aset_{\per(\theta)}} \Rg(\alg, \theta)$ be the instance dependent lower bound with the minimax optimality constraint. Then we have
\begin{proposition}
\begin{align*}
\tilde{\Rg}_{\per}(\theta) = 
\begin{cases}
\theta^* - \theta_{1:n}^* & \textrm{ if } \theta_{1:n}^* > \theta_{n:k+1}^{-} \\
0 & \textrm{ otherwise}. 
\end{cases}
\end{align*}
\end{proposition}

\begin{proof}
...
\end{proof}

$\alg_0$ is instance-wise optimal with respect to $\tilde{\Rg}_{\per}$~(and also $\Rper$) on most of the instances
\begin{proposition}
Define $\Thetat=\left\{ \theta: \theta_{1:n}^* > \theta_{n+1:k}^- \right\}$. 
Then $\sup_{\theta \in \Thetat} \frac{\Rg(\alg_{0}, \theta)}{\tilde{\Rg}_{\per}(\theta)} = 1$.
%Then For $n\le k-2$, $\sup_{\theta \in \Thetat} \frac{\Rg(\alg_{\alpha}, \theta)}{\tilde{\Rg}_{\per}(\theta)} = \frac{1}{1 - \alpha}$. For $n=k-1$, $\sup_{\theta \in \Thetat} \frac{\Rg(\alg_{\alpha}, \theta)}{\tilde{\Rg}_{\per}(\theta)} = \max\{ \frac{\alpha}{ 1 - \alpha}, 1\}$.
\end{proposition}

\begin{proof}
...
\end{proof}

Unlike $\Radv$, here we have a stronger argument on why $\alg_0$ might be more favorable when compared to $\tilde{\Rg}_{\per}$. That is, under any permutation invariant prior distribution over $\Theta$, $\alg_0$ minimizes the probability that the ratio between the actual regret and $\tilde{\Rg}_{\per}(\theta)$ is unbounded among all index algorithms. 
\begin{proposition}
For $n\le k-2$, let $\cP$ be any permutation invariant distribution over $\Theta$ and $\cP(\exists i\ne j, \theta_i=\theta_j)=0$~($\theta$ does not contain duplication entries almost surely). Then we have
\todoy[inline]{The following result might be inexact, needs to be double checked.}
\begin{align*}
\lefteqn{\cP\left(\frac{\Rg(\alg_{\alpha}, \theta)}{\tilde{\Rg}_{\per}(\theta)} = +\infty \right)} \\
= &\frac{n}{k}\cP(\theta^* < \alpha) + \frac{n!(k-n-1)!(k-n-1)}{k!} 
\end{align*}
where we define $0/0=1$.
\end{proposition}

\begin{proof}
...
\end{proof}

\todoy[inline]{Replace $+\infty$ with a constant $c\ge 1$ will give a more complete picture and may be more realistic (does not require the observed data to contain the optimal action.) But might be a bit complicated.}
\todoy[inline]{Derive $|\Thetat|$ under the uniform distribution over $\Theta$.}
\todoy[inline]{Try to prove similar results in the stochastic setting.}

\todoy[inline]{A separate question: Is there a notion of ``data dependent optimality'' (i.e. given observations, the algorithm minimize the worst case regret among all possible~(or most) instances)? This should automatically justify the optimality
of pessimism in the deterministic setting. In the stochastic setting, pessimistic algorithms can be approximately viewed as optimizing the quantile of posterior regret/reward given a  (uniform?) prior. The question is that whether we should be satisfied with this type of optimality, and why~(and maybe this is something that we may want to discuss as well).}


==> instance_upper.tex <==
\newpage

\section*{Instance dependent upper bounds}

\todoy[inline]{Attempting to get a tighter upper bound...}




\begin{theorem}
Consider index algorithms where $\idx_i = \hat{\mu}_i + b_i$ and $\cA(X) = \argmax_i \idx_i$.
For each $2\le i\le k$, define
\begin{align*}
g_i(\eta) =  \sum_{j\ge i} e^{-\frac{n_j}{2} \left(\eta - \mu_j - b_j\right)_+ ^2}
+ \min_{j < i} e^{-\frac{n_j}{2} \left(\mu_j + b_j - \eta \right)_+ ^2}
\end{align*}
and $g_i^* = \min_{\eta} g_i(\eta)$. Assuming $\mu_1\ge \mu_2\ge...\ge\mu_k$, we have
\begin{align*}
\Prb{\cA(X)\ge i} \le \min\{ 1, g_i^* \}  \addeq\label{eq:ub-cdf-general}
\end{align*}
and
\begin{align*}
\cR(\cA) \le \sum_{2\le i \le k} \Delta_i \left(\min\{ 1, g_i^* \} - \min\{ 1, g_{i+1}^* \} \right) \addeq\label{eq:ub-exp-general}
\end{align*}
where we define $g_{k+1}^*=0$.
\label{thm:instance-upper-general}
\end{theorem}

\todoy[inline]{
Why do we care about this? This is actually bounding the CDF of the regret and takes all factors into account instead of having $\Delta_{\max}, \Delta_{\min}, n_1, n_{\min}$, etc. 
One advantage is that the upper bound derived in this way, e.g. for LCB, will not depend on $n_1$ to be large. The bound for LCB is small whenever there exists $i$ such that $\Delta_i$ is small and $n_i$ is large, thus more ``instance dependent'' and closer to the practical situation (and the actual performance), e.g. we do not need to see the optimal action but a near-optimal action is enough.
}




Note that \eqref{eq:ub-cdf-general} and \eqref{eq:ub-exp-general} is already a well defined bound 
on the CDF and expected regret although not quite interpretable. Next we will instantiate the bound for 
specific choices of index functions $\idx_i = \hat{\mu}_i + b_i$.


\begin{corollary}[Worst-case for any index algorithm.]
Consider any index algorithm where $\idx_i = \hat{\mu}_i + b_i$, $\cA(X) = \argmax_i \idx_i$,
and $b_i  \in \left[ - \sqrt{\frac{2}{n_{i}}\log\frac{k}{\delta}}, \sqrt{\frac{2}{n_{i}}\log\frac{k}{\delta}} \right]$ for all $i\in \iset{k}$. We have
\begin{align*}
\mu^* - \mu_{\cA(X)}  \le   \sqrt{\frac{32}{n_{\min}}\log\frac{k}{\delta}}
\end{align*}
with probability at least $1 - \delta$ for any $\theta$.
\label{coro:ub-worst-case}
\end{corollary}
\todoy[inline]{Convert to bound in expectation?}



\begin{corollary}[Upper bound for LCB.]
Consider the LCB algorithm where $\idx_i = \hat{\mu}_i - \sqrt{\frac{2}{n_{i}}\log\frac{k}{\delta}}$ and $\cA(X) = \argmax_i \idx_i$. We have
\begin{align*}
\mu^* - \mu_{\cA(X)}  \le \min_{i\in \iset{k}} \Delta_i + \sqrt{\frac{8}{n_{i}}\log\frac{k}{\delta}}
\end{align*}
with probability at least $1 - \delta$.
\label{coro:ub-lcb-instance}
\end{corollary}

\todoy[inline]{This may not be the most refined bound for LCB from Theorem~\ref{thm:instance-upper-general} but the form looks clean and interpretable. e.g., This is tighter than picking $i=1$ in the upper bound.~(same for the bounds for other algorithms)}





\begin{corollary}[Upper bound for Greedy.]
Consider the Greedy algorithm where $\cA(X) = \argmax_i \hat{\mu}_i$. 
% Define $h^* = \argmin_{i\in \iset{k}} \Delta_i + \sqrt{\frac{2}{n_{i}}\log\frac{k}{\delta}} $.
We have
\begin{align*}
& \mu^* - \mu_{\cA(X)}  \\
& \le  \min_{i\in \iset{k}} \left(\Delta_{i} + \sqrt{\frac{2}{n_{i}}\log\frac{k}{\delta}} + \max_{j>i} \sqrt{\frac{2}{n_{j}}\log\frac{k}{\delta}} \right)
\end{align*}
with probability at least $1 - \delta$.
\label{coro:ub-greedy-instance}
\end{corollary}




\begin{corollary}[Upper bound for UCB.]
Consider the UCB algorithm where $\idx_i = \hat{\mu}_i + \sqrt{\frac{2}{n_{i}}\log\frac{k}{\delta}}$ and $\cA(X) = \argmax_i \idx_i$. We have
\begin{align*}
\mu^* - \mu_{\cA(X)}  \le \min_{i \in \iset{k}} \left( \Delta_i + \max_{j > i} \sqrt{\frac{8}{n_{j}}\log\frac{k}{\delta}} \right)
\end{align*}
with probability at least $1 - \delta$.
\label{coro:ub-ucb-instance}
\end{corollary}

\todoy[inline]{
Compare these bounds, LCB v.s. UCB might be interesting.
Propose arguments according to upper bounds
Verify these arguments through experiments.
Use the permutation model to explain why LCB might be more favorable in general (requires $k$ to be large.)
}


\newpage

\section*{Proof for upper bounds}

\begin{proof}[Proof of Theorem~\ref{thm:instance-upper-general}]

Assuming $\mu_1\ge \mu_2 \ge ,...,\mu_k$. If we can bound
$\Prb{\cA(X)\ge i} \le B_i$ where $B_1=1 \ge B_2 \ge...\ge B_k$. Then we can write
\begin{align*}
\cR(\cA) & = \sum_{2\le i \le k} \Delta_i \Prb{\cA(X)=i} \\
& = \sum_{2\le i \le k} \Delta_i \left( \Prb{\cA(X)\ge i} - \Prb{\cA(X) \ge i + 1}\right) \\
& = \sum_{2 \le i \le k} \left(\Delta_i - \Delta_{i-1}\right) \Prb{\cA(X)\ge i} \\
& \le \sum_{2 \le i \le k} \left(\Delta_i - \Delta_{i-1}\right) B_i \\
& = \sum_{2\le i \le k} \Delta_i (B_i - B_{i+1}) \,.
\end{align*}



To upper bound $\Prb{\cA(X)\ge i}$, let $\idx_i$ be the index for algorithm $\cA$, i.e., $\cA(X) = \argmax_i \idx_i$. Then
\begin{align*}
\Prb{\cA(X)\ge i} \le \Prb{\max_{j\ge i} \idx_j \ge \max_{j<i} \idx_j} \,.
\end{align*}

\todoy[inline]{How to bound this tightly?}

We can further write 
\begin{align*}
\Prb{\cA(X)\ge i} 
& \le \Prb{\max_{j\ge i} \idx_j \ge \max_{j<i} \idx_i, \max_{j<i} \idx_j \ge \eta} \\
& + \Prb{\max_{j\ge i} \idx_j \ge \max_{j<i} \idx_i, \max_{j<i} \idx_j < \eta} \\
& \le  \Prb{\max_{j\ge i} \idx_j \ge \eta} + \Prb{\max_{j<i} \idx_j < \eta}
\,.  \addeq\label{eq:ub-eta}
\end{align*}
Then optimize the choice of $\eta$ according to the design of $\idx$. e.g. greedy, LCB, UCB, ... etc.

We consider index algorithms where $\idx_i = \hat{\mu}_i + b_i$.

Continue with~\eqref{eq:ub-eta}, for the first term, by union bound we have 
\begin{align*}
\Prb{\max_{j\ge i} \idx_j \ge \eta}  \le \sum_{j\ge i} \Prb{\idx_j \ge \eta}  \,.
\end{align*}
For each $j\ge i$, by Hoeffding's inequality we have 
\begin{align*}
\Prb{\idx_j \ge \eta} \le e^{-\frac{n_j}{2} \left(\eta - \mu_j - b_j\right)_+ ^2} \,.   
\end{align*}
For the second term in~\eqref{eq:ub-eta}, we have $\Prb{\max_{j<i} \idx_j < \eta} \le \Prb{\idx_j < \eta}$ 
for each $j < i$.

By Hoeffding's inequality we have 
\begin{align*}
\Prb{\idx_j \ge \eta} \le  e^{-\frac{n_j}{2} \left(\mu_j + b_j - \eta \right)_+ ^2} \,.   
\end{align*}
So we have 
\begin{align*}
 \Prb{\max_{j<i} \idx_j < \eta} \le \min_{j<i} e^{-\frac{n_j}{2} \left(\mu_j + b_j - \eta \right)_+ ^2} \,.
\end{align*}
Define
\begin{align*}
g_i(\eta) =  \sum_{j\ge i} e^{-\frac{n_j}{2} \left(\eta - \mu_j - b_j\right)_+ ^2}
+ \min_{j < i} e^{-\frac{n_j}{2} \left(\mu_j + b_j - \eta \right)_+ ^2}
\end{align*}
and $g_i^* = \min_{\eta} g_i(\eta)$, we have
\begin{align*}
\Prb{\cA(X)\ge i} \le \min\{ 1, g_i^* \} \,. 
\end{align*}
Then we can bound the expected regret as
\begin{align*}
\cR(\cA) \le \sum_{2\le i \le k} \Delta_i \left(\min\{ 1, g_i^* \} - \min\{ 1, g_{i+1}^* \} \right)
\end{align*}
where we define $g_{k+1}^*=0$.

\todoy[inline]{Need to show $g_i^*$ is monotonic? should be easy}

\end{proof}


\begin{proof}[Proof of Corollary~\ref{coro:ub-worst-case}]
Let $\eta = \mu_1 - 2 \sqrt{\frac{2}{n_{\min}}\log\frac{k}{\delta}}$ and apply Theorem~\ref{thm:instance-upper-general}.

More specifically, we can show
\begin{align*}
g_i^* \le  \sum_{j\ge i} e^{-\frac{n_{\min}}{2} \left(\Delta_j - 3 \sqrt{\frac{2}{n_{\min}}\log\frac{k}{\delta}} \right)_+ ^2} + \frac{\delta}{k}
\end{align*}
then only consider $i$ such that $\Delta_i \ge 4\sqrt{\frac{2}{n_{\min}}\log\frac{k}{\delta}}$.


\todoy[inline]{finish the proof..}
\end{proof}


\begin{proof}[Proof of Corollary~\ref{coro:ub-lcb-instance}]
Let $\eta = \max_i \mu_i -  \sqrt{\frac{8}{n_i}\log\frac{k}{\delta}}$ and apply Theorem~\ref{thm:instance-upper-general}. We only consider $i$ where $\Delta_i > \mu_1 - \eta$.

Considering the LCB algorithm,
for each $i\ge 2$,
\begin{align*}
g_i(\eta) =  & \sum_{j\ge i} e^{-\frac{n_j}{2} \left(\eta - \mu_j + \sqrt{\frac{2}{n_j}\log\frac{k}{\delta}} \right)_+ ^2} \\
& + \min_{j < i} e^{-\frac{n_j}{2} \left(\mu_j - \eta - \sqrt{\frac{2}{n_j}\log\frac{k}{\delta}} \right)_+ ^2} \,.
\end{align*}

Define $h_i = \argmax_{j<i} \mu_j - \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}}$ and $\eta_i =\mu_{h_i} - \sqrt{\frac{8}{n_{h_i}}\log\frac{k}{\delta}}$. Then we have
$
e^{-\frac{n_{h_i}}{2} \left(\mu_{h_i} - \eta_i - \sqrt{\frac{2}{n_j}\log\frac{k}{\delta}} \right)_+ ^2} = \delta/k
$.
Consider $j \ge i$ we have 
\begin{align*}
e^{-\frac{n_j}{2} \left(\eta_i - \mu_j + \sqrt{\frac{2}{n_j}\log\frac{k}{\delta}}\right)_+ ^2} \le \frac{\delta}{k}
\end{align*}
whenever $\eta_i - \mu_j \ge 0$, i.e. $\mu_{h_i} - \sqrt{\frac{8}{n_{h_i}}\log\frac{k}{\delta}} \ge \mu_j$.

Define
\begin{align*}
U_i = \I{\forall j \ge i, \mu_{h_i} - \sqrt{\frac{8}{n_{h_i}}\log\frac{k}{\delta}} \ge \mu_j } \,.
\end{align*}
Then we have
$
g_i^* U_i \le \frac{k - i + 2}{k}\delta \le \delta
$.
According to Theorem~\ref{thm:instance-upper-general} we have $\Prb{\cA(X)\ge i} \le \min\{ 1, g_i^* \}$,
so for any $i$ such that $\Prb{\cA(X)\ge i} > \delta$, we must have $U_i = 0$, which is equivalent to 
\begin{align*}
\mu_i > \max_{j<i} \mu_j - \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}}\,.
\addeq\label{eq:proof-lcb-cond-1}
\end{align*}
Let $\hat{i}$ be the maximum $i$ that satisfies \eqref{eq:proof-lcb-cond-1}. 
Then we have $\Prb{\cA(X)\ge \hat{i} + 1} \le \delta$. Therefore, we have $\Prb{\mu^* - \mu_{\cA(X)} \le \Delta_{\hat{i}}} \ge 1 - \delta$. So it remains to upper bound $\Delta_{\hat{i}}$.

For any $i \in \iset{k}$, if $\hat{i} \le i$ then $\Delta_{\hat{i}} \le \Delta_{i}$. If $\hat{i} > i$ we have 
\begin{align*}
\mu_{\hat{i}} > \max_{j < \hat{i}} \mu_j - \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}}  \ge \mu_i - \sqrt{\frac{8}{n_i}\log\frac{k}{\delta}} \,.
\end{align*}
Therefore,
\begin{align*}
\Delta_{\hat{i}} = \Delta_i + \mu_{i} - \mu_{\hat{i}} \le \Delta_i + \sqrt{\frac{8}{n_{i}}\log\frac{k}{\delta}} \,,
\end{align*}
 which concludes the proof.

\if0
Pick $\eta=\mu_1$ then the second term in $g_i(\eta)$ becomes $\delta/k$. For $j$ such that $\Delta_j\ge \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}}$ we have 
\begin{align*}
e^{-\frac{n_j}{2} \left(\eta - \mu_j - \sqrt{\frac{2}{n_j}\log\frac{k}{\delta}} \right)_+ ^2} \le \frac{\delta}{k} \,.
\end{align*}
Define
\begin{align*}
U_i = \I{\forall j \ge i, \Delta_j\ge \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}} } \,.
\end{align*}
Then we have
$
g_i^* U_i \le \frac{k - i + 2}{k}\delta \le \delta
$.
According to Theorem~\ref{thm:instance-upper-general} we have $\Prb{\cA(X)\ge i} \le \min\{ 1, g_i^* \}$,
so for any $i$ such that $\Prb{\cA(X)\ge i} > \delta$, we must have $U_i = 0$, which is equivalent to 
\begin{align*}
\max_{j \ge i} \mu_j + \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}} > \mu_1\,.
\addeq\label{eq:proof-ucb-cond-1}
\end{align*}

For any $i \in \iset{k}$, if $\hat{i} \le i$ then $\Delta_{\hat{i}} \le \Delta_{i}$. If $\hat{i} > i$ we have 
\begin{align*}
\max_{j \ge \hat{i}} \mu_j + \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}}  \le \mu_{\hat{i}} + \max_{j > i} \sqrt{\frac{8}{n_{j}}\log\frac{k}{\delta}} \,.
\end{align*}
Applying \eqref{eq:proof-ucb-cond-1} gives
\begin{align*}
\Delta_{\hat{i}} = \mu_{1} - \mu_{\hat{i}} \le \max_{j > i} \sqrt{\frac{8}{n_{j}}\log\frac{k}{\delta}} \,.
\end{align*}
Therefore,
\begin{align*}
\Delta_{\hat{i}} 
& \le \max\left\{ \Delta_{i}, \max_{j > i} \sqrt{\frac{8}{n_{j}}\log\frac{k}{\delta}} \right\} \\
& \le \Delta_{i} + \max_{j > i} \sqrt{\frac{8}{n_{j}}\log\frac{k}{\delta}} \,.
\end{align*}
for any $i \in \iset{k}$, which concludes the proof.
\fi


\end{proof}





\begin{proof}[Proof of Corollary~\ref{coro:ub-greedy-instance}]
Considering the greedy algorithm,
for each $i\ge 2$,
\begin{align*}
g_i(\eta) =  \sum_{j\ge i} e^{-\frac{n_j}{2} \left(\eta - \mu_j\right)_+ ^2}
+ \min_{j < i} e^{-\frac{n_j}{2} \left(\mu_j - \eta \right)_+ ^2} \,.
\end{align*}
Define $h_i = \argmax_{j<i} \mu_j - \sqrt{\frac{2}{n_j}\log\frac{k}{\delta}}$ and $\eta_i =\mu_{h_i} - \sqrt{\frac{2}{n_{h_i}}\log\frac{k}{\delta}}$. Then we have
$
e^{-\frac{n_{h_i}}{2} \left(\mu_{h_i} - \eta_i \right)_+ ^2} = \delta/k.
$.
Consider $j \ge i$ we have 
\begin{align*}
e^{-\frac{n_j}{2} \left(\eta_i - \mu_j\right)_+ ^2} = e^{-\frac{n_j}{2} \left(\mu_{h_i} - \mu_j - \sqrt{\frac{2}{n_{h_i}}\log\frac{k}{\delta}} \right)_+ ^2} \,.
\end{align*}

When $\mu_{h_i} - \mu_j \ge \sqrt{\frac{2}{n_{h_i}}\log\frac{k}{\delta}} + \sqrt{\frac{2}{n_{j}}\log\frac{k}{\delta}}$ we have $e^{-\frac{n_j}{2} \left(\eta_i - \mu_j\right)_+ ^2} \le \delta/k$.

Define 
\begin{align*}
U_i = \I{\forall j \ge i, \mu_{h_i} - \mu_j \ge \sqrt{\frac{2}{n_{h_i}}\log\frac{k}{\delta}} + \sqrt{\frac{2}{n_{j}}\log\frac{k}{\delta}}} \,.
\end{align*}
Then we have
$
g_i^* U_i \le \frac{k - i + 2}{k}\delta \le \delta
$.
According to Theorem~\ref{thm:instance-upper-general} we have $\Prb{\cA(X)\ge i} \le \min\{ 1, g_i^* \}$,
so for any $i$ such that $\Prb{\cA(X)\ge i} > \delta$, we must have $U_i = 0$, which is equivalent to 
\begin{align*}
\max_{j<i} \mu_j - \sqrt{\frac{2}{n_{j}}\log\frac{k}{\delta}} < \max_{j \ge i} \mu_j  + \sqrt{\frac{2}{n_{j}}\log\frac{k}{\delta}} 
\addeq\label{eq:proof-greedy-cond-1}
\end{align*}
Let $\hat{i}$ be the maximum $i$ that satisfies \eqref{eq:proof-greedy-cond-1}. 
Then we have $\Prb{\cA(X)\ge \hat{i} + 1} \le \delta$. Therefore, we have $\Prb{\mu^* - \mu_{\cA(X)} \le \Delta_{\hat{i}}} \ge 1 - \delta$. So it remains to upper bound $\Delta_{\hat{i}}$.

For any $i \in \iset{k}$, if $\hat{i} \le i$ then $\Delta_{\hat{i}} \le \Delta_{i}$. If $\hat{i} > i$ we have 
\begin{align*}
\max_{j<\hat{i}} \mu_j - \sqrt{\frac{2}{n_{j}}\log\frac{k}{\delta}} \ge \mu_{i} - \sqrt{\frac{2}{n_{i}}\log\frac{k}{\delta}}
\end{align*}
and
\begin{align*}
\max_{j \ge \hat{i}} \mu_j  + \sqrt{\frac{2}{n_{j}}\log\frac{k}{\delta}} \le \mu_{\hat{i}} + \max_{j > i} \sqrt{\frac{2}{n_{j}}\log\frac{k}{\delta}} \,.
\end{align*}
applying \eqref{eq:proof-greedy-cond-1} gives
\begin{align*}
\Delta_{\hat{i}} - \Delta_{i} = \mu_{i} - \mu_{\hat{i}} \le \sqrt{\frac{2}{n_{i}}\log\frac{k}{\delta}} +  \max_{j > i} \sqrt{\frac{2}{n_{j}}\log\frac{k}{\delta}} \,.
\end{align*}
So
\begin{align*}
\Delta_{\hat{i}} \le \Delta_{i} + \sqrt{\frac{2}{n_{i}}\log\frac{k}{\delta}} +  \max_{j > i} \sqrt{\frac{2}{n_{j}}\log\frac{k}{\delta}} \,.
\end{align*}
for any $i \in \iset{k}$, which concludes the proof.




\end{proof}





\begin{proof}[Proof of Corollary~\ref{coro:ub-ucb-instance}]
Considering the UCB algorithm,
for each $i\ge 2$,
\begin{align*}
g_i(\eta) =  & \sum_{j\ge i} e^{-\frac{n_j}{2} \left(\eta - \mu_j - \sqrt{\frac{2}{n_j}\log\frac{k}{\delta}} \right)_+ ^2} \\
& + \min_{j < i} e^{-\frac{n_j}{2} \left(\mu_j - \eta + \sqrt{\frac{2}{n_j}\log\frac{k}{\delta}} \right)_+ ^2} \,.
\end{align*}
Pick $\eta=\mu_1$ then the second term in $g_i(\eta)$ becomes $\delta/k$. For $j$ such that $\Delta_j\ge \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}}$ we have 
\begin{align*}
e^{-\frac{n_j}{2} \left(\eta - \mu_j - \sqrt{\frac{2}{n_j}\log\frac{k}{\delta}} \right)_+ ^2} \le \frac{\delta}{k} \,.
\end{align*}
Define
\begin{align*}
U_i = \I{\forall j \ge i, \Delta_j\ge \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}} } \,.
\end{align*}
Then we have
$
g_i^* U_i \le \frac{k - i + 2}{k}\delta \le \delta
$.
According to Theorem~\ref{thm:instance-upper-general} we have $\Prb{\cA(X)\ge i} \le \min\{ 1, g_i^* \}$,
so for any $i$ such that $\Prb{\cA(X)\ge i} > \delta$, we must have $U_i = 0$, which is equivalent to 
\begin{align*}
\max_{j \ge i} \mu_j + \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}} > \mu_1\,.
\addeq\label{eq:proof-ucb-cond-1}
\end{align*}
Let $\hat{i}$ be the maximum $i$ that satisfies \eqref{eq:proof-ucb-cond-1}. 
Then we have $\Prb{\cA(X)\ge \hat{i} + 1} \le \delta$. Therefore, we have $\Prb{\mu^* - \mu_{\cA(X)} \le \Delta_{\hat{i}}} \ge 1 - \delta$. So it remains to upper bound $\Delta_{\hat{i}}$.

For any $i \in \iset{k}$, if $\hat{i} \le i$ then $\Delta_{\hat{i}} \le \Delta_{i}$. If $\hat{i} > i$ we have 
\begin{align*}
\max_{j \ge \hat{i}} \mu_j + \sqrt{\frac{8}{n_j}\log\frac{k}{\delta}}  \le \mu_{\hat{i}} + \max_{j > i} \sqrt{\frac{8}{n_{j}}\log\frac{k}{\delta}} \,.
\end{align*}
Applying \eqref{eq:proof-ucb-cond-1} gives
\begin{align*}
\Delta_{\hat{i}} = \mu_{1} - \mu_{\hat{i}} \le \max_{j > i} \sqrt{\frac{8}{n_{j}}\log\frac{k}{\delta}} \,.
\end{align*}
Therefore,
\begin{align*}
\Delta_{\hat{i}} 
& \le \max\left\{ \Delta_{i}, \max_{j > i} \sqrt{\frac{8}{n_{j}}\log\frac{k}{\delta}} \right\} \\
& \le \Delta_{i} + \max_{j > i} \sqrt{\frac{8}{n_{j}}\log\frac{k}{\delta}} \,.
\end{align*}
for any $i \in \iset{k}$, which concludes the proof.

\end{proof}



\newpage

==> mom.tex <==
\newcommand{\bnorm}[1]{\left\Vert #1\right\Vert}
\newcommand{\TV}[1]{\left\Vert #1\right\Vert_{\textrm{TV}}}

\subsection{Proof of \cref{thm:mom}} \todot{I will clean this up and make the proof consistent with the statement (just constants need to change).}
Let $\theta \in \Theta_n$ be an instance and abbreviate $[A, B] = I(X)$, so that $A$ and $B$ are random variables.
Let $m$ and $\alpha \max_a \mu_a$ be such that
\begin{align*}
\sum_{a=1}^k 1\left(\mu_a + \Delta_a \geq \alpha\right) = m\,.
\end{align*}
where $\Delta_a = \sqrt{\log(\epsilon m)/n_a}$ for suitably chosen $\epsilon \in (0,1)$ to be chosen subsequently.
To simplify the notation, assume without loss of generality that the arms are ordered in a such a way that
\begin{align*}
\mu_a + \Delta_a \geq \alpha \text{ for all } a \leq m\,.
\end{align*}
Given $b \in [m]$, let $\mu^b \in \RR^k$ be the vector with
\begin{align*}
\mu^b_a =
\begin{cases}
\mu_a & \text{if } a \neq b \\
\mu_a + \Delta_a & \text{otherwise}\,.
\end{cases}
\end{align*}
Then, by the assumption on validity, for any $a \in [m]$, $\sP_a(B \geq \alpha) \geq 1 - \delta$, which implies that
\begin{align*}
\sP(B \geq \alpha) 
&\geq \frac{1}{m} \sum_{a=1}^m \sP_a(B(X) \geq \alpha) - \TV{\sP - \frac{1}{m} \sum_{a=1}^m P_a} 
\geq 1 - \delta - \TV{\sP - \frac{1}{m} \sum_{a=1}^m \sP_a}\,,
\end{align*}
where $\TV{\cdot}$ is the usual total variation norm.
Letting $\sP' = \frac{1}{m} \sum_{a=1}^m \sP_a$ and $\epsilon \in (0,1)$, the
total variation distance satisfies
\begin{align*}
\TV{\sP - \sP'}
&= \EE\left[\left(1 - \frac{d \sP'}{d \sP}\right) 1\left(\frac{d \sP'}{d \sP} \leq 1\right)\right] 
\leq 1 - \frac{4}{5} \sP\left(\frac{d \sP'}{d \sP} \geq \frac{4}{5} \right) \,.
\end{align*}
Let $\bar M = \frac{1}{m} \sum_{a=1}^m M_a$ with
\begin{align*}
M_a = \exp\left(\frac{n_a}{2}\left((\hat \mu_a - \mu_a)^2 - (\hat \mu_a - \tilde \mu_a)^2\right)\right)
= \exp\left(n_a \Delta_a (\hat \mu_a - \mu_a) - \frac{n_a \Delta_a^2}{2}\right)\,.
\end{align*}
Then, by the Payley-Zygmund inequality and the fact that $\EE[M_a] = 1$, 
\begin{align*}
\sP\left(\frac{d \sP'}{d \sP} \geq \frac{4}{5}\right)
&= \sP\left(\bar M \geq  \frac{4}{5} \EE[\bar M] \right) 
\geq \frac{\EE[\bar M]^2/25}{\Var[\bar M] + \EE[\bar M]^2/25} \\
&= \frac{1/25}{\EE[\Var \bar M] + 1/25} 
= \frac{1/25}{1/25 + \frac{1}{m^2} \sum_{a=1}^m \Var(M_a)}
\end{align*}
Note that $M_a$ has a log-normal distribution and hence $\Var[M_a] = \exp(n_a \Delta_a^2) - 1$.
Therefore,
\begin{align*}
\sP\left(\frac{d \sP'}{d \sP} \geq \frac{4}{5}\right)
\geq  \frac{1/25}{1/25 + \frac{1}{m^2} \sum_{a=1}^m \exp(n_a \Delta_a^2)} 
\geq \frac{15}{16}\,.
\end{align*}
where in the final inequality we chose $\Delta_a = \sqrt{\log(c m) / n_a}$ for suitable constant $c > 0$.
Therefore $\TV{\sP - \sP'} \leq 1/4$, which implies that
\begin{align*}
\sP(B \geq \alpha) \geq \frac{3}{4} - \delta \,.
\end{align*}
For the lower bound, let $\alpha$ be as stated and let $\mu'$ be the vector of means with
\begin{align*}
\mu'_b =
\begin{cases}
\alpha &\text{if } \mu_b \geq \alpha \\
\mu_b &\text{otherwise}\,.
\end{cases}
\end{align*}
Since the maximum mean of $\mu'$ is $\alpha$, as before, by the validity of the algorithm,
\begin{align*}
\sP'(A(X) \geq \alpha) \leq \delta\,.
\end{align*}
On the other hand, the relative entropy between $\sP$ and $\sP'$ satisfies 
\begin{align*}
\KL(\sP, \sP') = \sum_{a=1}^k n_a (\mu_a - \mu'_a)^2 / 2 \leq 1 \,.
\end{align*}
Since $\TV{\sP - \sP'} \leq \sqrt{\KL(\sP, \sP')/2}$,
\begin{align*}
\sP(A \leq \alpha) \geq \sP'(A \leq \alpha) - \TV{\sP - \sP'} \geq 1 - \delta - \sqrt{1/2}\,.
\end{align*}
Naive simplification and a union bound shows that
\begin{align*}
\sP(I \subset [a(\theta), b(\theta)]) \geq \frac{1}{25} - \delta\,,
\end{align*}
which yields the result.


